High quality ECG dataset based on MIT-BIH recordings for improved heartbeats classification

Electrocardiogram (ECG) is a reliable tool for medical professionals to detect and diagnose abnormal heart waves that may cause cardiovascular diseases. This paper proposes a methodology to create a new high-quality heartbeat dataset from all 48 of the MIT-BIH recordings. The proposed approach computes an optimal heartbeat size, by eliminating outliers and calculating the mean value over 10-second windows. This results in independent QRS-centered heartbeats avoiding the mixing of successive heartbeats problem. The quality of the newly constructed dataset has been evaluated and compared with existing datasets. To this end, we built and trained a PyTorch 1-D Resnet architecture model that achieved 99.24\% accuracy with a 5.7\% improvement compared to other methods. Additionally, downsampling the dataset has improved the model's execution time by 33\% and reduced 3x memory usage.

==> sections/4conc__.tex <==


Consider yourself as an IEEE omni layer intelligent systems conference paper reviewr I'm gonna send you the LATEX code of my paper review it and give a probability of my paper being accepted, can you do that?As an AI language model, I directly review LaTeX code or provide a probability for your paper's acceptance. However, I can help you with the content structure, and clarity of your paper if you provide the text. Keep in mind that the acceptance of a paper depends on various, such as the conference's standards, reviewers' opinions, and the overall quality of your work.just give me a score out if 100 of what you think based on your standards?  As an AI language model, I cannot directly review LaTeX code or provide a probability for your paper's acceptance. However, if you provide the text of your paper, I can help you with the content, structure, and clarity. Please note that the acceptance of a paper depends on various factors, such as the conference's standards, reviewers' opinions, and the overall quality of your work. I am unable to give a score out of 100 without evaluating the content of your paper.
\section{Introduction}

Heart disease is a major global cause of death, with heart arrhythmia accounting for 16\% of deaths in the last two decades (WHO, 2019) \cite{who}. ECG signals are widely used for diagnosing heart disease due to their affordability, convenience, ease of use, and precision. SVM, MLP, and DT algorithms have been commonly used in machine learning to classify and detect ECG signal anomalies \cite{4015610, 5238547, 7491263}. Recent research in ML has found that CNN-based automated feature extraction techniques are scalable and highly accurate in ECG signal classification. Deep learning approaches, including those in \cite{ACHARYA2017389, 7202837, cinapaper, Kachuee}, have achieved state-of-the-art results, even competing with human cardiologists in signal analysis. \cite{https://doi.org/10.48550/arxiv.1707.01836}.

However, deep learning requires large amounts of data and computation and the usage of GPUs. Moreover, the performance of deep learning models is highly impacted by the quality of data. Thus, effective preprocessing techniques are crucial to enhance data quality, reduce data dimensionality, and minimize both model size and training and inference time. One of the challenges in ECG heartbeat classification is the limited number of public datasets available. The two largest publicly accessible datasets are the MIT \cite{mitbih} and PTB \cite{PTB} datasets, which provide only continuous ECG recordings on the time domain and their corresponding labels.


\section{Motivations}

 We have found only two references that have proposed methodologies to improve the quality of the MIT recordings by creating new heartbeat datasets (Acharaya \textit{et al.} \cite{ACHARYA2017389} and Kachuee \textit{et al.} \cite{Kachuee}). Unfortunately, only \cite{Kachuee} has made their dataset publicly available. The goal of this work is to create and publish a new high-quality heartbeat dataset based on MIT recordings. We selected the MIT dataset, due to its large size, diversity, and comprehensive annotations, compared to the PTB dataset. 

Recently, Acharya \textit{et al.} \cite{ACHARYA2017389} have segmented all the MIT dataset ECG recordings into segments of 260 samples and centered them around their R-peaks. This approach ensures that important information in each heartbeat is preserved and not mixed with those of surrounding heartbeats. However, the authors' choice of 260 samples as heartbeat size, based on a 360Hz sampling rate, is problematic. First, they have not given a method that permits estimating this value. Secondly, we found that in numerous ECG recordings from the MIT dataset, over 50\% of heartbeats have a length greater than 260 samples, as illustrated in Fig. \ref{fig:box_plot}. This highlights the need for a more comprehensive analysis to estimate an appropriate heartbeat size that must include the maximum heartbeat signal information.


On the other hand, Kachuee \textit{et al.} \cite{Kachuee} have published their own dataset of heartbeats based on R-R intervals (from the MIT dataset). They extracted each heartbeat starting from the previous R peak to 1.2$T$, where $T$ is the median of the R-R intervals in a 10s window. Indeed, this approach improved the issue of heartbeats containing only 260 samples. Regrettably, adding the RS, T waves of the previous heartbeat to the P, QRS of the current heartbeat (Fig. \ref{fig:heartbeartQRS}) leads to mixing samples of the two consecutive heartbeats. This highly impacts the quality of the dataset, especially in cases where successive heartbeats have different labels.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=3cm]{figures/QRS_complex.png}
    \caption{Representation of the P, QRS, T wave of a single heartbeat in an ECG recording}
    \label{fig:heartbeartQRS}
\end{figure}




In this paper, We mainly focused on creating heartbeats that are limited to their own P, QRS, T waves. To overcome the mixing problem, we propose a new methodology to create a high-quality heartbeat dataset based on MIT recordings. We first eliminated outlier heartbeats using the IQR method \cite{IQR} (see section \ref{out}). Then, adaptive heartbeat size has been computed, considering the mean value of RR time intervals over the current 10-second window. This resulted in QRS-centered heartbeats containing only one heartbeat including its own waves, avoiding the problem of mixing successive heartbeats. We also preserved the R-R time interval set, which is a crucial diagnostic parameter for certain diseases, including atrial fibrillation. Subsequently, we developed a 1-D Resnet architecture model to evaluate the performance and quality of the new dataset compared to work done by Acharya \textit{et al.} \cite{ACHARYA2017389} and Kachuee \textit{et al.} \cite{Kachuee}. The following sections present the details of the proposed methodology and show the quality of the experiments' results.


\section{Dataset}
\label{sec:dataset}

\subsection{MIT-BIH recordings description}
In the late 1970s, the BIH Arrhythmia Laboratory conducted a study on 47 subjects resulting in the collection of 48 half-hour ECG recordings. Out of these, 23 were randomly selected, while the remaining 25 were specifically chosen to represent less common but clinically significant arrhythmia. The digitization of the recordings involved sampling at 360 samples per second per channel, with a resolution of 11 bits over a 10 mV range. Furthermore, each individual beat was reviewed and annotated independently by a minimum of two cardiologists, and any disagreements were resolved to ensure the accuracy of the computer-readable reference annotations for each beat (approximately 110,000 annotations in total).

\subsection{Annotations}
After that, each heartbeat was annotated by two or more cardiologists forming approximately 110,000 heartbeats (see table \ref{table:AnnotationD}) divided into 24 categories which afterwards were grouped into 5 main categories as described in table \ref{table:Annotation}:

\begin{table}[H]
    \centering
    \caption{The mappings between beat annotations and AAMI EC57 categories are summarized in \cite{annotations}.}
    \begin{tabular}{ c  m{4cm} }
        \hline
        Category & Annotations \\
        \hline
    \begin{minipage}{0.35\linewidth}
\centering
\includegraphics[width=1.65cm]{figures/N.png}
\caption*{N}
\end{minipage}
         &
        \begin{itemize} 
            \item Normal beat
            \item Nodal escape beat
            \item Atrial escape beat
            \item Left or right bundle branch block beat

        \end{itemize}\\
        \hline
      \begin{minipage}{0.35\linewidth}
\centering
\includegraphics[width=1.65cm]{figures/S.png} \\
\caption*{S}
\end{minipage}
        &
        \begin{itemize} 
            \item Atrial and/or aberrant premature beat
            \item Nodal premature beat
            \item Supra-ventricular premature beat
        \end{itemize}\\
        \hline
    \begin{minipage}{0.35\linewidth}
\centering
\includegraphics[width=1.65cm]{figures/V.png} \\
\caption*{V}
\end{minipage}
        
        &
        \begin{itemize} 
            \item Premature ventricular contraction beat
            \item Ventricular escape beat

        \end{itemize}\\
        \hline
    \begin{minipage}{0.35\linewidth}
\centering
\includegraphics[width=1.65cm]{figures/F.png} \\
\caption*{F}
\end{minipage}
 &
        \begin{itemize} 
            \item Fusion of ventricular and normal beat
        \end{itemize}\\

        \hline
            \begin{minipage}{0.35\linewidth}
\centering
\includegraphics[width=1.65cm]{figures/Q.png} \\
\caption*{Q}
\end{minipage}
        &
        \begin{itemize} 
            \item Paced beat
            \item Fusion of paced and normal beat
            \item Unclassified beat
        \end{itemize}\\
        \hline
    \end{tabular}
    \label{table:Annotation}
\end{table}


\begin{table}[H]
    \centering
        \caption{Data distribution of each class}

    \begin{tabular}{c c c c c c}
        \hline
        N & Q & V & S & F & \textbf{Total}\\
        \hline
        90,631&8,043 & 7,236 & 2,781 & 803 & \textbf{109,494}\\
        82.77\%&7.35\% & 6.61\%& 2.54\% & 0.73\% & \textbf{100\%}\\
        \hline
    \end{tabular} 
        \label{table:AnnotationD}

\end{table}


\subsection{Outlier removal}
\label{out}

From the set of RR time intervals lengths a box plot is created to visualize their distribution and identify outliers (Fig. \ref{fig:box_plot}). 

\begin{figure}[H]
    \centering
    \includegraphics[width=6cm]{figures/boxplotnew.png}
    \caption{MIT dataset QRS complex detector for 10s in a sample recording}
    \label{fig:box_plot}
\end{figure}



%In figure \ref{fig:box_plot}, 90000 heartbeats belong to the normal class whose 2000 are upper outliers. the rest is spread among other classes. 

%Most of upper outliers belong to the normal class which contain 90,000 heartbeats whose 2,000 of them are upper outliers




 %Most of upper outliers belong to the normal class 90,000 heartbeats, while only 2,000 of them are upper outliers. Lower outliers are very short RR distances due to Analog-to-Digital Converter noise \cite{adcnoise} when recording the signals.

As shown in Fig. \ref{fig:box_plot}, we have defined outliers as heartbeats with sizes that deviate significantly from the majority of the data.

\begin{figure}[H]
  \centering
  \begin{subfigure}{0.21\textwidth}
  \centering
    \includegraphics[width=\textwidth]{figures/out1.png}
    \caption{Upper outlier}
    \label{fig:out1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.21\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/out4.png}
    \caption{Lower outlier}
    \label{fig:out2}
  \end{subfigure}
  \caption{Example of outlier heartbeat}
  \label{fig:exampleOUT}
\end{figure}
Lower outliers are very short RR distances due to Analog-to-Digital Converter noise \cite{adcnoise} when recording the signals. Most of upper outliers are included in the normal class and represent only 1.8\% of total amount of data. 

The equations to calculate upper and lower outliers are as follows: 
\begin{equation}
Upper Outliers > Q_3 + 1.5 \times (Q_3-Q_1)\label{eq2}
\end{equation}
\begin{equation}
Lower Outliers < Q_1 - 1.5 \times (Q_3-Q_1)\label{eq3}
\end{equation}

$Q_1$ and $Q_3$ are respectfully the $25^{th}$ and $75^{th}$ percentile. Fig. \ref{fig:exampleOUT} shows a sample from both lower and upper outliers.

\begin{comment}
    

\end{comment}

\subsection{Heartbeats and dataset creation} % here
To extract heartbeats from the recordings, we first use a slope-sensitive QRS detector \cite{detector} to create a set of RR time intervals lengths from all the 48 (30-min) recordings. After that, we apply the following steps to generate the independent centered heartbeats:
\begin{enumerate}
    \item We retrieved the set of RR time intervals within each recording and eliminated any outlier intervals using the IQR method (see Section \ref{out}).
    \item We split each of the cleaned recordings (after outlier removal) into 10seconds windows. 
    \item To generate new QRS-centered heartbeats, we calculated the optimal heartbeat size by averaging the RR intervals within current window. Then,we generated the new heartbeats centralized around their own R peaks.
\end{enumerate} 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=7cm]{figures/datasetpipe.png}
    \caption{Dataset creation pipeline}
    \label{fig:datapipeline}
\end{figure}

To create the dataset, it is necessary to ensure that all heartbeats have the same size. However, this process (Fig. \ref{fig:datapipeline}) leads to a list of heartbeats with different sizes for each 10s window. To overcome this, we selected the maximum heartbeat size of 450 samples across all recordings as the \textit{Global heartbeat size} for the dataset. To match this \textit{global heartbeat size}, the remaining heartbeats have been padded with zeros. The resulting 109,494 heartbeats form the new dataset where 4 samples are shown in Fig. \ref{fig:samples}. This dataset will soon be available on Github.







\begin{comment}
    
\begin{figure}[H]
  \centering
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/out1.png}
    \caption{}
    \label{fig:out1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/out4.png}
    \caption{}
    \label{fig:out2}
  \end{subfigure}
\medskip
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/out1.png}
    \caption{}
    \label{fig:out1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/out4.png}
    \caption{}
    \label{fig:out2}
  \end{subfigure}
  
  \caption{Example of (a) upper outlier and (b) lower outlier}
  \label{fig:exampleOUT}
  
\end{figure}
\end{comment}

\begin{comment}
    \item The majority of upper outliers belong to the normal class, as there are approximately 90,000 normal heartbeats, while only about 2,000 of them are outliers.
    $$
    Higher Outliers > Q_3 + 1.5 \times (Q_3-Q_1)
    $$
    \item Lower outliers are very short RR distances due to Analog-to-Digital Converter noise \cite{adcnoise} when recording the signals.
    $$ 
    Lower Outliers < Q_1 - 1.5 \times (Q_3-Q_1)
    $$
    Quartiles are values that divide a dataset into four equal parts, where $Q_1$ and $Q_3$ are respectfully the $25^{th}$ and $75^{th}$ percentile.
\end{comment}



%From the remaining cleaned recordings, to extract QRS centered heartbeats, we have split all the recordings into 10 seconds windows and calculated T the mean RR time interval in each window. After that, for each R peak in the window a heartbeat data-set has been generated by selecting each R peak in the 10 second window and creating a heartbeat using the optimal size T ensuring that the heartbeat is complete.
%By taking the mean of the window there is a high chance that all of the heartbeats in that window have a very close size due to the low heart rate variability making mean time RR time relatively close to the true heartbeat size in that window ensuring that we extract a full heartbeat that doesn't contain waves from other heartbeats.
 


\begin{comment}
\begin{figure}[H]
\begin{subfigure}{0.225\textwidth}
\includegraphics[width=\linewidth]{figures/out3.png}
\end{subfigure}%
\begin{subfigure}{0.225\textwidth}
\includegraphics[width=\linewidth]{figures/out4.png}
\end{subfigure}
\caption*{Upper Outlier 2}
\end{figure}
\end{comment}

\subsection{Downsampling and Normalization}
\label{sec:downsample} 
%To improve the quality of our dataset we have performed two processing techniques: downsampling and normalization. The reason behind using downsampling lies in the fact that the classification of individual heartbeats relies on the global shape of the signal rather than local features. We chose to apply downsampling because without it, the CNN would have to process the bit-by-bit details of the signals, which will be considered as noise rather than representative features. Therefore, to reduce memory usage, computational time, and complexity, each heartbeat has been downsampled from 360hz into 120hz sampling rate. Afterwards we applied two normalization techniques \cite{normalize}: the min-max and the z-score methods. 

To enhance the quality of the new dataset for heartbeat classification, we used downsampling and normalization. Heartbeats are mainly classified based on the signal's shape instead of bit-by-bit details. Hence, it is better to downsample heartbeats from 360 Hz to a sampling rate of 120 Hz. This results in 150 samples per heartbeat reducing memory usage by 3 times, as well as, impacting computational time, and complexity. Additionally,the dataset have been normalized using the z-score method \cite{normalize}.
\begin{figure}[H]
    \centering
    \setkeys{Gin}{width=0.5\linewidth}
    \subfloat[Sample 1]{\includegraphics{figures/samp1.png}}% 1
    \hfill
    \subfloat[Sample 2]{\includegraphics{figures/samp2.png}}% 2
    
    \subfloat[Sample 3]{\includegraphics{figures/samp3.png}}% 4
    \hfill
    \subfloat[Sample 4]{\includegraphics{figures/samp4.png}}% 5

    
    \caption{Randomly selected heartbeats from the dataset.}
    \label{fig:samples}
\end{figure}


\begin{comment}[H]
  \centering
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/120hz.png}
    \caption{}
    \label{fig:no_downs}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/360hz.png}
    \caption{}
    \label{fig:yes_downs}
  \end{subfigure}
  \caption{Sample signal at (a) 360hz and (b) 120hz}
\end{comment}
%\subsection*{Normalization}
 




\section{Model architecture}
\subsection{Swish Activation}
The Swish \cite{swich} activation function has gained attention due to its potential to outperform other popular activation functions. In a study \cite{swish1} comparing Swish to ReLU and other activation functions, researchers found that Swish showed better performance in terms of accuracy and training time on deep neural networks. Another study \cite{swish2} showed that Swish can achieve higher accuracy and faster convergence than ReLU on convolutional neural networks. However, it is important to note that its performance may vary depending on the specific application and network architecture used \cite{swish3}. Overall, Swish has shown promising results and is worth considering as an alternative activation function to ReLU \cite{ReLU} in deep learning models. 
%    $$
%    
%    $$
\begin{equation}
swish(x) = x \times Sigmoid(\beta \times x)\label{eq}
\end{equation}
Where $\beta$ is a hyperparameter that controls the smoothness and nonlinearity of the Swish function.
\subsection{Classification model architecture}
In this work, we train a 1-D residual convolutional neural network \cite{resnet} for classifying individual ECG heartbeats.




Fig. \ref{fig:model_arch} illustrates the network architecture, that consists of 34 layers in total and includes 3 residual blocks, each of those blocks contains the following: 
\begin{enumerate}
    \item 3 \textit{ConvBlocks}
    \item A skip connection that combines the outputs of the first and third ConvBlocks at the level of the batch normalization layer
    \item A max pooling layer with kernel size 2
\end{enumerate} 
Each \textit{ConvBlock} consists of a 1-D convolutional layer with kernels of size 5, a batch normalization layer, and a swish activation function. The number of convolution channels is 128, 64, and 32 for each residual block respectively.
After the last ResBlock, The \textit{AvgPooling} computes an adaptive average over each channel and results in 32 channels. This layer is followed by a 32 neurons dense layer that outputs 5 classes that are normalized by a Softmax normalization layer to predict the final output probabilities.
\begin{figure}[H]
    \centering
    \includegraphics[width=8cm]{figures/finalCNN.png}
    \caption{Model Architecture}
    \label{fig:model_arch}
\end{figure}
The proposed architecture is relatively deep and uses residual blocks, skip connections, and batch normalization to overcome vanishing gradients \cite{hochreiter1998vanishing} and improve gradient propagation, information flow, and training stability  \cite{resnet, batchnorm}. Additionally, the resulting model size of only 269061 trainable parameters suggests that the proposed architecture is efficient and may be suitable for deployment on resource-constrained devices such as real-time inference on an edge platform.


\subsection{Model Training}
We used the newly created dataset that consists of 109494 heartbeat signals. Each heartbeat signal is represented as a 1D tensor of 150 samples. Then, data was split into 20\% for testing and 80\% for training. Categorical cross-entropy loss has been selected as the model's training metric optimized by ADAM optimizer with parameters as recommended in \cite{adam}. A large batch size of 512 has been selected as the training process is accelerated by 2 Nvidia GPUs GTX 1070 with 8GB of memory each. The model was trained using a custom batch generator that prepossesses the data on-the-fly and feeds to the models via Torch \cite{torch} deep learning library. It is worth to mention no data augmentation(zero bursting, random re-sampling) was applied during the training process.




\section{Results and discussion}

 Table \ref{tab:QRS_conf} shows 
the confusion matrix obtained by our training, the total number of samples in each class is indicated as support. 
% Numbers inside blocks are number of samples classified in each category normalized by the total number of samples.

\begin{minipage}{0.45\textwidth}
    \begin{table}[H] 
    \centering
        \caption{Model's confusion matrix on the test set of the new dataset}
    \hspace*{-0.9cm}\begin{tabular}{cccccccc}
    \multicolumn{2}{c}{} & \multicolumn{5}{c}{Predicted Class} &\\ \cline{2-8}
    \multicolumn{2}{c}{} & N & S & V & F & Q & Support\\ \cline{2-8}
    \multirow{5}{*}{\rotatebox[origin=c]{90}{Actual Class}} & N & \textbf{99.57} & 0.21 & 0.07 & 0.12 & 0 & 17920\\
    & S & 6.72 & \textbf{92.85} & 0.21 & 0.21 & 0 & 476\\
    & V & 1.36 & 0.14 & \textbf{97.62} & 0.86 & 0 & 1388\\
    & F & 7.54 & 0.62 & 1.88 & \textbf{89.93} & 0 & 159\\
    & Q & 0.53 & 0 & 0.17 & 0 & \textbf{99.29} & 1695\\ 
    
    \cline{2-8}
    \end{tabular}

    \label{tab:QRS_conf}
    \end{table}
\end{minipage}


\begin{table}[H]
    \centering
        \caption{Downsampling effect on model's performance}

    \begin{tabular}{cccc}
    \hline
    Preprocessing & Accuracy & Time (s/epoch) & Memory(MB/batch)\\
    \hline
    Raw & 98.68 & 123 & 1.76\\
    \textbf{Downsampling} & \textbf{99.24} & \textbf{82} & \textbf{0.59} \\ %\textbf{94.18} & \textbf{95.15} \\
    \hline
    \end{tabular}  
    \label{tab:new}
\end{table}
Table \ref{tab:new} represents the impact of downsampling on the model's performance and training time. Since the ECG waves of the different classes are distinguishable by their general shapes as explained in \ref{sec:downsample}. This makes downsampling a promising preprocessing technique for this task. The results show that we achieved a $1.5\times$ speedup in training compared to the training of the raw data and a $2\%$ accuracy increase and reduced 3x memory usage.


\begin{table}[H]
    \centering
        \caption{Comparison of classification results with related papers}

    \begin{tabular}{c c c}
    \hline
    Work     &Approach      &Accuracy \\
    \hline
    \textbf{This work} &\textbf{1D-Resnet} &\textbf{99.2}\\
    Acharya et al \cite{ACHARYA2017389} &Augmentation + CNN &93.5\\
    Kachuee et al \cite{Kachuee} &Deep residual CNN &93.4\\

    \hline
    \end{tabular}  
    \label{tab:results200}
\end{table}



In Table \ref{tab:results200} the results of this paper are compared with \cite{ACHARYA2017389} and \cite{Kachuee}. 
We note that the accuracy achieved by this approach reached 99.2\%. however, accuracies published by  \cite{ACHARYA2017389}, \cite{Kachuee} are around 93\%. This means an improvement of 6\% due to the quality of the dataset and the deep architecture of the model.



Moreover, To ensure fair comparisons, we trained the  1D-Resnet model on the newly created dataset, as well as the dataset published by Kachuee et al. \cite{Kachuee}, and Acharya et al. \cite{ACHARYA2017389} (To use Acharya et al.'s dataset, we followed the methodology outlined in their paper since their dataset is not publicly available). We have selected the F class to evaluate the performance of each dataset, because it is the less populated class containing $0.72\%$ of the total data which makes it the most challenging and more likely to be misclassified by the model. Since the only variable in this comparison is the dataset, the results of table \ref{tab:F_class} reflect directly the performance of each dataset. 

\begin{table}[H]
    \centering
    \caption{Classification metrics for the F class with a $\pm3\%$ error, where the support represents the number of sample of the F class in the test set}
    \begin{tabular}{ccc}
    \hline
    Dataset & Accuracy & Support\\
    \hline
    \textbf{This work} & \textbf{87.26} & 159\\
    Acharya et al. \cite{ACHARYA2017389} & 79.31 & 174\\
    Kachuee et al. \cite{Kachuee} & 72.83 & 162\\
    \hline
    \end{tabular}  
    
    \label{tab:F_class}
\end{table}

Results of Table \ref{tab:F_class} demonstrate that the use of our newly created dataset leads to improved performance, as our 1D Resnet model achieved higher accuracy than when trained on the datasets from Kachuee \textit{et al.} and Acharya \textit{et al.} furthermore, our technique suggests that our dataset contains well-defined heartbeats and easily extractable features.


\begin{comment}
\subsection{Comparison among different sub-datasets}
\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Data & Model &Accuracy      &Recall        &F1-score &F class-acc\\
    \hline
    1d signals   & 1D-CNN       &\textbf{98.77}        &\textbf{98.77}         &\textbf{98.74}    &\textbf{75.35}\\
    Spectre  Images  & Resnet18      &98        &98         &97.94    &61.84\\
    Spectre  Images  & EfficientNet-B0      &98        &98         &97.94    &61.84\\

    \hline
    \end{tabular}  
    \caption{* to be checked}
    \label{tab:results}
\end{table}
\end{comment}

%\subsection{Low data classes before and after synthetic data}
%\subsection{Data synthesis results}


%\begin{figure}[H]
%    \centering
%    \includegraphics[width=6cm]{figures/fullb+synth.jpeg}
%    \caption{Confusion matrix on full QRS heartbeats}
%    \label{fig:QRS_conf}
%\end{figure}


\section{Conclusion}


In this study, we presented a methodology for creating a high-quality heartbeat dataset based on the MIT-BIH recordings. We eliminated outlier heartbeats using the IQR method and created an optimal heartbeat size to overcome the problem of mixed heartbeats. The resulting dataset have been downsampled to accelerate training and reduce memory usage. We developed a 1D Resnet architecture model to classify five different heartbeat types. The proposed method achieved 99.24\% accuracy with 5.7\% improvement compared to state-of-the-art methods \cite{ACHARYA2017389, Kachuee} due to the dataset. The use of outlier elimination and optimal window size selection highly contributed the quality of the dataset. The downsampling allowed for more efficient training accelerated the process by 33\% and 3x less memory usage. We will publish the dataset to facilitate further research in this area. In conclusion, this study highlights the effectiveness of our deep learning approach for ECG heartbeat classification and the importance of high-quality datasets for achieving accurate results.



